Sketched Gaussian Mechanism for Private Federated Learning

Communication cost and privacy are two major considerations in federated learning (FL). For communication cost, gradient compression by sketching the clients' transmitted model updates is often used for reducing per-round communication. For privacy, the Gaussian mechanism (GM), which consists of clipping updates and adding Gaussian noise, is commonly used to guarantee client-level differential privacy. Existing literature on private FL analyzes privacy of sketching and GM in an isolated manner, illustrating that sketching provides privacy determined by the sketching dimension and that GM has to supply any additional desired privacy. In this paper, we introduce the Sketched Gaussian Mechanism (SGM), which directly combines sketching and the Gaussian mechanism for privacy. Using R\'enyi-DP tools, we present a joint analysis of SGM's overall privacy guarantee, which is significantly more flexible and sharper compared to isolated analysis of sketching and GM privacy. In particular, we prove that the privacy level of SGM for a fixed noise magnitude is proportional to $1/\sqrt{b}$, where $b$ is the sketching dimension, indicating that (for moderate $b$) SGM can provide much stronger privacy guarantees than the original GM under the same noise budget. We demonstrate the application of SGM to FL with either gradient descent or adaptive server optimizers, and establish theoretical results on optimization convergence, which exhibits only a logarithmic dependence on the number of parameters $d$. Experimental results confirm that at the same privacy level, SGM based FL is at least competitive with non-sketching private FL variants and outperforms them in some settings. Moreover, using adaptive optimization at the server improves empirical performance while maintaining the privacy guarantees.

==> arxiv_SGM/sections/convergence_analysis.tex <==
In this section, we will analyze the optimization performance of the differentially private sketching federated learning algorithm described in Algorithm \ref{alg:fed_sgm}. First, in Section \ref{subsec:asmp}, we will state our assumptions on loss gradients and Hessian spectrum and explain why they are well-supported by previous works. Then in Section \ref{subsec:optimization}, we will demonstrate optimization results of Algorithm \ref{alg:fed_sgm} with gradient descent and AMSGrad as the \texttt{GLOBAL\_OPT}. 
\subsection{Assumptions}\label{subsec:asmp}
We begin by presenting a set of standard assumptions that are widely adopted in the literature on first-order stochastic methods.
\begin{asmp}[Bounded Loss Gradients]\label{asmp:gradient_norm}
There exists a constant $G \geq 0$, such that for every $\left(\mathbf{x},y\right)$, $\left\|\nabla \ell(\theta;(x,y))\right\|_{2} \le G$.
\label{asmp:bcg}
\end{asmp}
According to the definition, the local (stochastic) gradient $g_{c,t,k}$ and $\nabla\mathcal{L}_{c}(\theta)$ are both average of loss gradient over samples, so we have $\left\|g_{c,t,k}\right\|_{2}\leq G$, $\left\|\nabla\mathcal{L}_{c}(\theta)\right\|_{2}\leq G$. Besides, $\nabla\mathcal{L}(\theta)=\frac{1}{C}\sum_{c=1}^{C}\nabla\mathcal{L}_{c}(\theta)$, so we can directly see that $\left\|\nabla\mathcal{L}(\theta)\right\|_{2}\leq G$. Therefore, $G$ is the upper bound for both the client and global gradient norms. We also assume the stochastic noise from minibatches is sub-Gaussian, which is widely adopted in first-order optimization~\citep{harvey2019tight,mou2020linear}.
\begin{asmp} [Sub-Gaussian Noise]\label{asmp:gradient_noise}
The stochastic noise $\left\|\nabla \cL_c(x) - g_{c}(x)\right\|_{2}$ at each client is a $\sigma_{s}$-sub-Gaussian random variable, i.e. $\P(\left\|\nabla \cL_{c}(x) - g_{c}(x)\right\|_{2} \ge a) \le 2 \exp(-a^2/\sigma_{s}^2)$, for all $a\ge 0$.
\label{asmp:local_grad_sub}
\end{asmp}
Besides, we also assume a special structure on the Hessian eigenspectrum $\{\lambda_i, v_i\}_{i=1}^d$ of the loss function $\ell$.
\begin{asmp} [Bounded Loss Hessian Eigenvalues]\label{asmp:smoothness}
The smoothness of the loss function $\ell$, i.e. the largest eigenvalue of the loss Hessian $H_\ell$ is bounded by $L$, $\max_i \lambda_i \le L$. 
\end{asmp}
The assumption on the boundedness of the loss Hessian $H_{\ell}$ is actually equivalent to the $L$-smoothness of the loss function $\ell$, which is commonly used in many federated learning analysis~\citep{safaryan2021fednl,fatkhullin2024momentum}. Due to a similar reason as Assumption \ref{asmp:gradient_norm}, this assumption also indicates the $L$-smoothness of the local loss function $\mathcal{L}_{c}$ and the average loss function $\mathcal{L}$.
\begin{asmp} [Loss Hessian Eigenspetrum]\label{asmp:hessian_eigen}
The absolute intrinsic dimension, which is defined as the ratio between the sum of absolute values and the largest eigenvalue of $H_{\mathcal{L}}$ eigenspectrum is bounded by $\mathcal{I}$, i.e., $\frac{\sum_{i=1}^{d}\left|\lambda_{i}\right|}{\max_{i}\lambda_{i}}\leq\mathcal{I}$.
\label{asmp:hessian_adaptive}
\end{asmp} 
The absolute intrinsic dimension considered here, $\frac{\sum_{i=1}^{d}\left|\lambda_{i}\right|}{\max_{i}\lambda_{i}}$, is close to the concept of intrinsic dimension proposed in \cite{ipsen2024stable}, and the difference is that we consider absolute values of eigenvalues. A growing amount of empirical research suggests that the absolute intrinsic dimension of the Hessian in deep learning can be significantly smaller than the ambient dimension $d$. Studies by \cite{ghorbani2019investigation, li2020hessian, liu2023sophia} indicate that the eigenspectrum undergoes a sharp decay in magnitude. Additionally, research by \cite{sagun2016eigenvalues, liao2021hessian} demonstrates that a substantial portion of the eigenspectrum is concentrated near zero. Further investigations by \cite{xie2022power, zhang2024transformers} reveal that the eigenvalues follow a power-law distribution, suggesting that in such cases, the absolute intrinsic dimension remains a much smaller order than $d$.
\subsection{Optimization Analysis}\label{subsec:optimization}
In this section, we will provide the optimization results of Algorithm \ref{alg:fed_sgm} with GD and AMSGrad as $\texttt{GLOBAL\_OPT}$.
\subsubsection{GD as \texttt{GLOBAL\_OPT}}\label{subsec:gd}
First we write down Algorithm \ref{alg:gd}, which will be called as \texttt{GLOBAL\_OPT} each round to do a one-step GD update of the global parameter $\theta_{t-1}$ with desketched aggregated updates $\desk\left(\bar{\tilde{\Delta}}_{t-1}\right)$.
\begin{algorithm}[h]
    {\bf Inputs:} model $\theta_{t-1}$, desketched update $\desk\left(\bar{\tilde{\Delta}}_{t-1}\right)$.\\
    {\bf Output:} model $\theta_{T}$.\\
    {\bf One-step GD:} $\theta_t \gets \theta_{t-1} - \eta_{\text{global}} \cdot \desk(\bar{\tilde{\Delta}}_{t-1})$.
    \caption{$\texttt{GLOBAL\_OPT}$ (GD)}
    \label{alg:gd}
\end{algorithm}
\vspace{-2mm}

Then we will introduce the optimization result of Algorithm \ref{alg:fed_sgm} with Algorithm \ref{alg:gd}. We follow a similar analysis to \cite{song2023sketching},
but we exploit the second order structure of the deep learning  losses, which helps avoid picking up dimension dependence due to the $\desk\left(\sk\left(\cdot\right)\right)$ operator. The formal version of result and all technical proofs are in Appendix \ref{proof:gd}.
\vspace{-1mm}
\begin{theorem}[Informal version of Theorem \ref{thm:gd_formal}]\label{thm:gd}
Suppose $\left\{\theta_{t}\right\}_{t=0}^{T}$ is generated by Algorithm \ref{alg:fed_sgm} with Algorithm \ref{alg:gd} as \texttt{GLOBAL\_OPT}. Denote $\mathcal{L^{*}}$ the minimum of the average empirical loss. Under Assumption \ref{asmp:gradient_norm}-\ref{asmp:hessian_eigen}, with learning rate $\eta=\eta_{\text{global}}\eta_{\text{local}}$, we have that with probability at least $1-\Theta\left(\delta\right)$,
\begin{align*}
    \frac{1}{T}\sum_{t=0}^{T-1}\left\|\nabla\mathcal{L}(\theta_{t})\right\|_{2}^{2}&\leq E^{\text{GD}}_{s}+E^{\text{GD}}_{c}+E^{\text{GD}}_{g}
\end{align*}
in which $E^{\text{GD}}_{s}$, $E^{\text{GD}}_{c}$ and $E^{\text{GD}}_{g}$ denote terms from sketching-based FedAvg algorithm, caused by clipping, and caused by Gaussian noises. Specifically,
\begin{align*}
    &E^{\text{GD}}_{s}=\frac{\mathcal{L}(\theta_{0})-\mathcal{L}^{*}}{\eta TK}+\tilde{\mathcal{O}}\left(\frac{1}{\sqrt{NT}}\right)+\tilde{\mathcal{O}}\left(\eta_{\text{local}}K\right)\\
    &+\tilde{\mathcal{O}}\left(\frac{\tau}{\sqrt{bT}K}\right)+\tilde{\mathcal{O}}\left(\frac{\eta\mathcal{I}\tau^{2}}{K}\right)+\tilde{\mathcal{O}}\left(\frac{1}{\eta TK}\right)\\
        %&E^{\text{GD}}_{s}=\frac{\mathcal{L}(\theta_{0})-\mathcal{L}^{*}}{\eta KT}+\frac{2\log(2T/\delta)G^{2}}{\sqrt{NT}}+\frac{\eta_{\text{local}}LKG^{2}}{2}\\
        %&+\frac{\sqrt{2}G\log(2T/\delta)\sigma_{s}}{\sqrt{NTK}}+\frac{\sqrt{2}\log^{2}(NTd/\delta)G\tau}{\sqrt{bT}K}+\frac{\eta\alpha_{1}^{2}\mathcal{I}L\tau^{2}}{K}\\
    &E^{\text{GD}}_{c}=\max\left\{0,\frac{G(KG-\tau)}{K}\right\}\\
    &E^{\text{GD}}_{g}=\tilde{\mathcal{O}}\left(\frac{\eta\mathcal{I}\sigma_{g}^{2}}{NK}\right)
        %&E^{\text{GD}}_{g}=\frac{\sqrt{2}\log^{2}(2T/\delta)\sigma_{g}G}{\sqrt{NT}K}+\frac{\eta\sigma_{g}^{2}\mathcal{I}L\log^{2}(2dT/\delta)}{NK}\\
        %&\alpha_{1}=1+\frac{\log^{1.5}(NTd^{2}/\delta)}{\sqrt{b}}
    \end{align*}
\end{theorem}
\begin{remark}\label{remark:gd_sketching_1}
Regarding the term $E^{\text{GD}}_{s}$, most of the optimization results for sketching-based algorithms are expectation results~\citep{song2023sketching,rothchild2020fetchsgd}, while ours is a high-probability optimization bound for the sketching-based FedAvg algorithm. In addition, previous optimization results in expectation either have a linear dependence on the ambient dimension $d$~\citep{song2023sketching}, or get around the dependence by using \texttt{Top-k} components of the gradient vector with rely on heavy-hitter assumptions~\citep{rothchild2020fetchsgd,zhang2024private}. As a contrast, our result $E^{\text{GD}}_{s}$ only has a logarithmic dimensional dependence from the need of high probability with no additional mechanisms.
\end{remark}
\begin{remark}\label{remark:gd_sketching_2}
When there is no clipping activated, i.e., $\tau=KG$, with learning rates $\eta_{\text{local}}=\mathcal{O}\left(\frac{\sqrt{\mathcal{I}}}{\sqrt{T}K}\right)$, $\eta=\mathcal{O}\left(\frac{1}{\sqrt{T\mathcal{I}}K}\right)$, we can get a convergence rate of $\tilde{\mathcal{O}}\left(\sqrt{\frac{\mathcal{I}}{T}}\right)$. When we clip with a constant, i.e., $\tau=\mathcal{O}(1)$, by setting $\eta_{\text{local}}=\mathcal{O}\left(\frac{1}{\sqrt{NT}K}\right)$, $\eta=\mathcal{O}\left(\frac{1}{\sqrt{T\mathcal{I}}}\right)$, the convergence rate becomes $\tilde{\mathcal{O}}\left(\frac{1}{\sqrt{NT}}+\frac{\sqrt{\mathcal{I}}}{\sqrt{T}K}\right)$.
%which is a slightly weaker but comparable result even to the standard FedAvg algorithm without sketching under partial worker participation~\citep{yang2021achieving}.
\end{remark}
\begin{remark}\label{remark:gd_clipping}
Regarding the term $E^{\text{GD}}_{c}$ caused by clipping, although in a high probability bound, we cannot obtain upper bounds with expression of gradients during training as in the expectation results~\citep{zhang2022understanding}, $\max\left\{0,\frac{G(KG-\tau)}{K}\right\}$ is still a reasonable term in the sense that it is monotonically decreasing with the clipping threshold $\tau$. In the extreme case, when $\tau=0$, all the clipped updates will become $0$, so that there is no training, then $E^{\text{GD}}_{c}=\max\left\{0,\frac{G(KG-\tau)}{K}\right\}=G^{2}$ is a natural bound of $\frac{1}{T}\sum_{t=0}^{T}\left\|\nabla\mathcal{L}(\theta_{t})\right\|_{2}^{2}=\left\|\nabla\mathcal{L}(\theta_{0})\right\|_{2}^{2}$ with Assumption \ref{asmp:gradient_norm}; when $\tau\geq KG$, there is no clipping activated during training, which is aligned with the fact that $E^{\text{GD}}_{c}=\max\left\{0,\frac{G(KG-\tau)}{K}\right\}=0$. 
\end{remark}
\begin{remark}\label{remark:gd_noise}
Regarding the term $E^{\text{GD}}_{g}$ caused by Gaussian noises, with the learning rates mentioned in Remark \ref{remark:gd_sketching_2}, $E^{\text{GD}}_{g}=\tilde{\mathcal{O}}\left(\frac{\sqrt{\mathcal{I}}\sigma_{g}^{2}}{N\sqrt{T}K}\right)$. Besides, $E^{\text{GD}}_{g}$ does not have any dependence on either the ambient dimension $d$ or the sketching dimension $b$.
\end{remark}
\subsubsection{AMSGrad as \texttt{GLOBAL\_OPT}}\label{subsec:amsgrad}
Similar to Section \ref{subsec:gd}, we will state Algorithm \ref{alg:amsgrad}, which will be used as \texttt{GLOBAL\_OPT} to do a one-step adaptive update of $\theta_{t-1}$ with $\desk\left(\bar{\tilde{\Delta}}_{t-1}\right)$.
\begin{algorithm}[ht]
    {\bf Inputs:} model $\theta_{t-1}$, desketched update $\desk\left(\bar{\tilde{\Delta}}_{t-1}\right)$.\\
    {\bf Output:} model $\theta_{T}$.\\
    {\bf Update first moment estimate:} $m_{t} = \beta_{1}m_{t-1}+(1-\beta_{1})\desk(\bar{\tilde{\Delta}}_{t-1})$\\
    {\bf Update second moment estimate:} $\hat{v}_{t} = \beta_{2}v_{t-1}+(1-\beta_{2})\left(\desk(\bar{\tilde{\Delta}}_{t-1})\right)^{2}$\\
    {\bf Update maximum of past second moment estimates:} $v_{t} = \max\left(\hat{v}_{t},v_{t-1}\right)$\\
    {\bf Update parameters:} $\theta_{t} = \theta_{t-1}-\eta_{\text{global}}\frac{m_{t-1}}{\sqrt{v_{t-1}}+\epsilon}:=\eta_{\text{global}}V_{t-1}^{-\frac{1}{2}}m_{t-1}$
    \caption{$\texttt{GLOBAL\_OPT}$ (AMSGrad)}
    \label{alg:amsgrad}
\end{algorithm}

Then we demonstrate the optimization result of Algorithm \ref{alg:fed_sgm} with Algorithm \ref{alg:amsgrad}. We
refer the reader to Appendix \ref{proof:amsgrad} for a more formal statement with the full analysis.
\begin{theorem}\label{thm:amsgrad}[Informal version of Theorem \ref{thm:amsgrad_formal}]
Suppose $\left\{\theta_{t}\right\}_{t=0}^{T}$ is generated by Algorithm \ref{alg:fed_sgm} with Algorithm \ref{alg:amsgrad} as \texttt{GLOBAL\_OPT}. Denote $\mathcal{L}^{*}$ the minimum of the average empirical loss. Under Assumption \ref{asmp:gradient_norm}-\ref{asmp:hessian_eigen}, with learning rate $\eta=\eta_{\text{global}}\eta_{\text{local}}$, we have that with probability at least $1-\Theta\left(\delta\right)$,
\begin{align*}
    \frac{1}{T}\sum_{t=0}^{T-1}\left\|\nabla\mathcal{L}\left(\theta_{t}\right)\right\|_{2}^{2}\leq E^{\text{AMSGrad}}_{s}+E^{\text{AMSGrad}}_{c}+E^{\text{AMSGrad}}_{g}
\end{align*}
in which $E^{\text{AMSGrad}}_{s}$, $E^{\text{AMSGrad}}_{c}$ and $E^{\text{AMSGrad}}_{g}$ denote terms from sketching-based FedAvg algorithm, caused by clipping, and caused by Gaussian noises. Specifically,
\begin{align*}
    &E^{\text{AMSGrad}}_{s}=\mathcal{O}\left(\frac{\mathcal{L}(\theta_{0})-\mathcal{L}^{*}}{\eta TK}\right)+\tilde{\mathcal{O}}\left(\frac{1}{\sqrt{NT}}\right)+\tilde{\mathcal{O}}\left(\eta_{\text{local}}K\right)\\
    &+\tilde{\mathcal{O}}\left(\frac{\tau}{\sqrt{bT}K}\right)+\tilde{\mathcal{O}}\left(\frac{\left(\eta_{\text{local}}+\eta\mathcal{I}\right)\tau^{2}}{K}\right)+\tilde{\mathcal{O}}\left(\frac{1}{\eta TK}\right)\\
    %&E^{\text{AMSGrad}}_{s}=\frac{\alpha_{2}\left(\mathcal{L}(\theta_{0})-\mathcal{L}^{*}\right)}{\eta KT}+\frac{2\alpha_{2}\log(2T/\delta)G^{2}}{\sqrt{NT}\epsilon}\\
    %&+\frac{\eta_{\text{local}}\alpha_{2}LKG^{2}}{2\epsilon}+\frac{\sqrt{2}\alpha_{2}G\log(2T/\delta)\sigma_{s}}{\sqrt{NTK}\epsilon}\\
    %&+\frac{\sqrt{2}\alpha_{2}\log^{2}(NTd/\delta)G\tau}{\sqrt{bT}K\epsilon}+\frac{\eta_{\text{local}}\alpha^{2}_{1}\alpha_{2}\sqrt{1-\beta_{2}}G\tau^{2}}{K\epsilon^{2}(1-\beta_{1})}\\
    %&+\frac{2\eta\alpha^{2}_{1}\alpha_{2}\left(1+2\beta_{1}\right)(1+\beta_{1})\mathcal{I}L\tau^{2}}{K\epsilon^{2}(1-\beta_{1})^{2}}\\
    &E^{\text{AMSGrad}}_{c}=\max\left\{0,\frac{\left(\epsilon+\tilde{\mathcal{O}}\left(\eta_{\text{local}}\right)\right)G(KG-\tau)}{K\epsilon}\right\}\\
    %E^{\text{AMSGrad}}_{c}&=\max\left\{0,\frac{\alpha_{2}G(KG-\tau)}{K\epsilon}\right\}\\
    &E^{\text{AMSGrad}}_{g}=\tilde{\mathcal{O}}\left(\frac{\left(\eta_{\text{local}}+\eta\mathcal{I}\right)\sigma_{g}^{2}}{NK}\right)%+\tilde{\mathcal{O}}\left(\frac{\eta_{\text{local}}\sigma_{g}^{2}}{NK}\right)
    %&E^{\text{AMSGrad}}_{g}=\frac{\eta_{\text{local}}\alpha_{1}\alpha_{2}(1+\beta_{1})\sqrt{1-\beta_{2}}G\tau\sigma_{g}\log(2dT/\delta)}{\sqrt{N}K\epsilon^{2}(1-\beta_{1})}\\
    %&+\frac{\eta_{\text{local}}\alpha_{2}\beta_{1}\sqrt{1-\beta_{2}}\sigma_{g}^{2}G\log^{2}(2dT/\delta)}{NK\epsilon^{2}(1-\beta_{1})}+\frac{\sqrt{2}\alpha_{2}\log^{2}(2T/\delta)\sigma_{g}G}{\sqrt{NT}K\epsilon}\\
    %&+\frac{2\eta\alpha_{2}(1+2\beta_{1})(1+\beta_{1})\sigma_{g}^{2}\mathcal{I}L\log^{2}(2dT/\delta)}{NK\epsilon^{2}(1-\beta_{1})^{2}}\\
    %&\alpha_{1}=1+\frac{\log^{1.5}(NTd^{2}/\delta)}{\sqrt{b}}\\  &\alpha_{2}=\eta_{\text{local}}\left(1+\frac{\log^{1.5}(NTd^{2}/\delta)}{\sqrt{b}}\right)\tau+\frac{\eta_{\text{local}}\sigma_{g}\log(2dT/\delta)}{\sqrt{N}}+\epsilon
\end{align*}
\end{theorem}
\begin{remark}\label{remark:amsgrad}
When we set the learning rates $\eta_{\text{global}}$ and $\eta_{\text{local}}$ as the same orders as Remark \ref{remark:gd_sketching_2}, we can see that both $E^{\text{AMSGrad}}_{s}$ and $E^{\text{AMSGrad}}_{g}$ are of the same orders as $E^{\text{GD}}_{s}$ and $E^{\text{GD}}_{g}$, and also exhibits only a logarithmic dependence on dimension arising solely from the requirement for high probability. Besides, under the learning rate selections with large enough $T$, $E_{c}^{\text{AMSGrad}}\approx\max\left\{0,\frac{G(KG-\tau)}{K}\right\}=E_{c}^{\text{GD}}$. Combining these three terms, it states that the performance of the differentially private sketching federated learning algorithm with AMSGrad as \texttt{GLOBAL\_OPT} is at least of the same level as with GD as \texttt{GLOBAL\_OPT}.
\end{remark}
\begin{remark}\label{remark:adaptive}
From the proof in Appendix \ref{proof:amsgrad}, we can see that our analysis on AMSGrad can be generated to any adaptive optimizers involved with first-order and second-order moments, including Adam~\citep{kingma2014adam}, Yogi~\citep{zaheer2018adaptive}, etc.
\end{remark}
%\begin{remark}\label{remark:amsgrad_sketching}
%Regarding the term $E^{\text{AMSGrad}}_{s}$, similar to $E_{s}^{\text{GD}}$, we also provide a high-probability optimization bound for the sketching-based adaptive federated learning algorithm. In addition, if we choose learning rates $\eta_{\text{global}}$ and $\eta_{\text{local}}$ as the same order of Remark \ref{remark:gd_sketching}, we can get the convergence rate of the same order $\mathcal{O}\left(\frac{1}{\sqrt{NT}}+\frac{1}{\sqrt{T}K}\right)$. And our $E^{\text{AMSGrad}}_{s}$ also does not have any dimensional dependence.
%\end{remark}
%\begin{remark}\label{remark:amsgrad_clipping}
%According to the definition of $\alpha_{2}$, we can see that when choosing the learning rate as in Remark \ref{remark:amsgrad_sketching}, $\alpha_{2}\approx\epsilon$ with large enough $T$. Therefore, $E_{c}^{\text{AMSGrad}}\approx\max\left\{0,\frac{G(KG-\tau)}{K}\right\}=E_{c}^{\text{gd}}$, which is a rational bound for clipping as stated in Remark \ref{remark:gd_clipping}.
%\end{remark}
%\begin{remark}
%Regarding the term $E^{\text{AMSGrad}}_{g}$ caused by Gaussian noises, with our learning rate setting in Remark \ref{remark:amsgrad_sketching}, we have $E^{\text{AMSGrad}}_{g}=\tilde{\mathcal{O}}\left(\right)$
%\end{remark}
The privacy-optimization trade-off can be evaluated by incorporating $\sigma_{g}^{2}$ from Theorem \ref{thm:dp_ma} into Theorem \ref{thm:gd} and Theorem \ref{thm:amsgrad}. To get deeper understanding on the impacts of hyperparameters, including $T$, $\eta$, $\eta_{\text{local}}$, on the trade-off, we consider the simplified situation in which $\tau\geq KG$ and $\sigma_{g}^{2}$ takes the lower bound. For the situation that $\tau<KG$, it will have an extra term caused by clipping, which is $E_{c}^{\text{GD}}$ for Theorem \ref{thm:gd} and $E_{c}^{\text{AMSGrad}}$ for Theorem \ref{thm:amsgrad}.
\begin{corollary}[Optimization with Privacy]
Assume all assumptions in Theorem \ref{thm:gd}/Theorem \ref{thm:amsgrad} hold. With the clipping threshold $\tau=c'K$ in which $c'\geq G$, $\left(\sigma_{g},b,\varepsilon_{p},\delta_{p}\right)$ satisfies the condition in Theorem \ref{thm:dp_ma}, $\eta=\mathcal{O}\left(\frac{1}{\sqrt{T\mathcal{I}}K}\right)$, $\eta_{\text{local}}=\mathcal{O}\left(\frac{\sqrt{I}}{\sqrt{T}K}\right)$, then we have Algorithm \ref{alg:fed_sgm} with Algorithm \ref{alg:gd} as \texttt{GLOBAL\_OPT} is $\left(\varepsilon_{p},\delta_{p}\right)$-differentially private, and with probability at least $1-\Theta\left(\delta\right)$,
\begin{align*}
    \frac{1}{T}\sum_{t=0}^{T-1}\left\|\nabla\mathcal{L}\left(\theta_{t}\right)\right\|_{2}^{2}\leq\underbrace{\tilde{\mathcal{O}}\left(\sqrt{\frac{\mathcal{I}}{T}}\right)}_{E_{s}}+\underbrace{\tilde{\mathcal{O}}\left(\frac{\sqrt{T\mathcal{I}}}{C^{2}\varepsilon_{p}^{2}}\right)}_{E_{g}}
\end{align*}
\end{corollary}
\begin{remark}
With the best selection of $T=\mathcal{O}\left(\frac{C^{2}\epsilon^{2}_{p}}{\log\frac{2}{\delta_{p}}}\right)$, we have
\vspace{-3mm}
\begin{align*}
    \frac{1}{T}\sum_{t=0}^{T-1}\left\|\nabla\mathcal{L}\left(\theta_{t}\right)\right\|_{2}^{2}\leq\tilde{\mathcal{O}}\left(\frac{\sqrt{\mathcal{I}}}{C\varepsilon_{p}}\right).
\end{align*}
\vspace{-5mm}
\end{remark}
\begin{remark}
Notice that the utility bound for the standard DP-SGD with the number of training samples $C$ and privacy level $\varepsilon_{p}$ is $\tilde{\mathcal{O}}\left(\frac{\sqrt{d}}{C\varepsilon_{p}}\right)$~\citep{bassily2014private, wang2022differentially,fang2023improved}. Our result is of the same order in terms of $\varepsilon_{p}$ and $C$, but rely on the absolute intrinsic dimension $\mathcal{I}$ defined in Assumption \ref{asmp:hessian_eigen}, which is much smaller than the ambient dimension $d$.
\end{remark}
